Language Model Decoding as Likelihood-Utility Alignment

A critical component of a successful language generation pipeline is the decoding algorithm. However, the general principles that should guide the choice of a decoding algorithm remain unclear. Previous works only compare decoding algorithms in narrow scenarios, and their findings do not generalize across tasks. We argue that the misalignment between the model's likelihood and the task-specific notion of utility is the key factor to understanding the effectiveness of decoding algorithms. To structure the discussion, we introduce a taxonomy of misalignment mitigation strategies (MMSs), providing a unifying view of decoding as a tool for alignment. The MMS taxonomy groups decoding algorithms based on their implicit assumptions about likelihood--utility misalignment, yielding general statements about their applicability across tasks. Specifically, by analyzing the correlation between the likelihood and the utility of predictions across a diverse set of tasks, we provide empirical evidence supporting the proposed taxonomy and a set of principles to structure reasoning when choosing a decoding algorithm. Crucially, our analysis is the first to relate likelihood-based decoding algorithms with algorithms that rely on external information, such as value-guided methods and prompting, and covers the most diverse set of tasks to date. Code, data, and models are available at https://github.com/epfl-dlab/understanding-decoding.

==> 12_figure2_1x4.tex <==
\begin{figure*}
     \centering
     
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/fig2/cIE_beam_search_5beams.pdf}
         \caption{REBEL}
         \label{fig:rebel_align_bs}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/fig2/Translation_beam_search.pdf}
         \caption{WMT14}
         \label{fig:wmt14_align_bs}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/fig2/Toxicity_beam_search.pdf}
         \caption{RTP}
         \label{fig:rtp_align_bs}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/fig2/Protein_beam_search.pdf}
         \caption{SwissProt}
         \label{fig:prot_align_bs}
     \end{subfigure}
     \caption{\textbf{RQ2}: For each dataset model pair, we run beam search and look into the $k=5$ final hypotheses and measure the correlation between likelihood and utility. As in \Figref{fig:fig1}, the y-axis is the task-specific utility score, and the x-axis is the model's log-likelihood (normalized for MT and cIE). The plots are generated as follows: (i) take the decoded outputs from \Figref{fig:fig1} from Beam Search with their (normalized) log-likelihood score and utility score, this indicates the x and y coordinate of each output, (ii) for each output look into the other hypotheses generated during beam search and compute among these hypotheses the Kendall's $\tau$ correlation between utility and log-likelihood, and (iii) average the correlation across all outputs within the same bin. 
     }
     \label{fig:fig2}
\end{figure*}
